Sparse Convolution for Approximate Sparse Instance

Computing the convolution $A \star B$ of two vectors of dimension $n$ is one of the most important computational primitives in many fields. For the non-negative convolution scenario, the classical solution is to leverage the Fast Fourier Transform whose time complexity is $O(n \log n)$. However, the vectors $A$ and $B$ could be very sparse and we can exploit such property to accelerate the computation to obtain the result. In this paper, we show that when $\|A \star B\|_{\geq c_1} = k$ and $\|A \star B\|_{\leq c_2} = n-k$ holds, we can approximately recover the all index in $\mathrm{supp}_{\geq c_1}(A \star B)$ with point-wise error of $o(1)$ in $O(k \log (n) \log(k)\log(k/\delta))$ time. We further show that we can iteratively correct the error and recover all index in $\mathrm{supp}_{\geq c_1}(A \star B)$ correctly in $O(k \log(n) \log^2(k) (\log(1/\delta) + \log\log(k)))$ time.

==> technique.tex <==
\section{Technique overview}


%\Zhao{Guangyi, please write at least 1.5 pages about technique overview.}

\iffalse
\subsection{approximate sparse non-negative convolution}

In this paper, we study the approximately $k$-sparse non-negative convolution problem and design an approximate sparse convolution algorithm (Algorithm~\ref{alg:approx_sparse_conv}) such that it can approximately recover the all index in $\supp_{\geq c_1}(A \star B)$ with point-wise error of $o(1)$ in $O(k \log (n) \log(k)\log(k/\delta))$ time.




Given we have two non-negative vectors, $A,B \in \R^n$, we want to compute $A \star B $ with probability $1-\delta$.

Assume there exist $c_1 = \Omega(1)$ and $c_2 = o(n^{-2})$ such that $\|A \star B\|_{\geq c_1} = k$ and $\|A \star B\|_{\leq c_2} = n-k$.

By using two properties of linear hashing basics in Lemma~\ref{lem:prime-hashing-basics}, with probability $1-\delta/k$ and Hoeffding bound in Lemma~\ref{lem:hoeffding}, we can prove that for all $i \in \supp_{\geq c_1}(A \star B)$, $i$ is isolated in at least $L/2$ hashing functions in $\{g^{(l)}\}_{l=1}^L$.
www

\subsection{iteratively correcting the errors}
\fi



